DrivingDiffusion: Layout-Guided multi-view driving scene video generation with latent diffusion model

With the increasing popularity of autonomous driving based on the powerful and unified bird's-eye-view (BEV) representation, a demand for high-quality and large-scale multi-view video data with accurate annotation is urgently required. However, such large-scale multi-view data is hard to obtain due to expensive collection and annotation costs. To alleviate the problem, we propose a spatial-temporal consistent diffusion framework DrivingDiffusion, to generate realistic multi-view videos controlled by 3D layout. There are three challenges when synthesizing multi-view videos given a 3D layout: How to keep 1) cross-view consistency and 2) cross-frame consistency? 3) How to guarantee the quality of the generated instances? Our DrivingDiffusion solves the problem by cascading the multi-view single-frame image generation step, the single-view video generation step shared by multiple cameras, and post-processing that can handle long video generation. In the multi-view model, the consistency of multi-view images is ensured by information exchange between adjacent cameras. In the temporal model, we mainly query the information that needs attention in subsequent frame generation from the multi-view images of the first frame. We also introduce the local prompt to effectively improve the quality of generated instances. In post-processing, we further enhance the cross-view consistency of subsequent frames and extend the video length by employing temporal sliding window algorithm. Without any extra cost, our model can generate large-scale realistic multi-camera driving videos in complex urban scenes, fueling the downstream driving tasks. The code will be made publicly available.

==> bucket.tex <==

%%%%% Comment start

\begin{comment}
\section{Method}
% Is this order proper?
 In this section, we elaborate the details of our method. Firstly, we introduce the overall architecture of our method. Second, we present the details of how to generate spatial keys and queries in our view-invariant cross attention. With those spatial items, our method can effectively learn the transformation from 2D image plane to 3D space in a view-invariant way. Then, we illustrate how we leverage the temporal frames to boost the performance. Finally, we introduce the heads and loss functions adopted in our method.
 
% Is this part needed ? The core is to explain the coordinate system here ?
% \subsection{Problem Definition}
% The aim of multi-view 3D object detection task is to detect 3D objects from multi-view RGB images. In general, the camera intrinsic and extrinsic parameters are also required as inputs in the process. Specifically, for each object, the location of objects' center$(cx, cy, cz)$, 3D dimensions$(w, h, l)$, orientation $\theta$ and the velocity$(vx, vy)$should be estimated in the global coordinate system. We denote the LiDAR coordinate system as the global system and camera coordinate system as the local system in this paper for better clarification. We also refer pixel coordinate system as the 2D local system.

\subsection{Overall Architecture}

The proposed method is an end-to-end imaged-based 3D object detector following~\cite{liu2022petr}. 
The overall architecture of \ourMethod{} consists of a CNN backbone, a transformer decoder and prediction heads. The CNN backbone extracts 2D multi-view features $F_{2d}\in \mathbb{R}^{S \times C \times H_F \times W_F}$ from images $I\in \mathbb{R}^{S \times 3 \times H_I \times W_I}$ in $S$ views. The transformer decoder aims to decode objects' location from object queries, which is stacked up with multiple layers. For each decoder layer, it is consists of five parts: a Key Feature-guided Position Encoder(KFPE) to generate spatial keys, a Query Feature-guided Position Encoder(KFPE) to generate spatial keys, a cross-attention layer, a self-attention layer and a feed-forward network layer. Both KFPE and QFPE are proposed to modulate the spatial items with content items.

\subsection{View-invariant Cross Attention}\label{subsection1}
\textbf{Review Cross Attention in PETR.} We first review the cross-attention mechanism in ~\cite{liu2022petr, liu2022petrv2}. The cross attention in PETR takes three inputs: queries, keys and values. Queries are generated from 3D reference points in global system with an attached small MLP network. Keys are formed by adding 2D features and 3D position embedding together. The 3D position embedding is further guided by image features in ~\cite{liu2022petrv2} to make the position embedding relevant with input. The values are composed of 2D image features. In this way, the transformation are learned from 2D image plane to 3D global space directly, which is rather complicate with big variance in camera extrinsics.



\textbf{Key Feature-guided Position Encoder.} 
In this part, we introduce how to generate the key position embedding in our cross attention. We firstly sample $D$ points along the axis orthogonal to the image plane with linear increasing depth values and generate a frustum $M_i \in \mathbb{R}^{D \times 3 \times H_F \times W_F}$ for each camera view. Then, we use re-project the camera frustum to the voxel in local system $V_i \in \mathbb{R}^{D \times 3 \times H_F \times W_F}$ for each view using only camera intrinsic parameters:
\begin{equation}
\begin{gathered}
V_i = I_i^{-1} M_i,
\end{gathered}
\end{equation}
where $i$ indicates the $i^{th}$ view. Next, we normalize the 3D coordinates of $V_i$ using the visible range in the $i^{th}$ local system to get $\overline{V_i}$. 

We encode the normalized 3D camera coordinates $\overline{V_i}$ to high-dimensional position encoding with a small convolution block $\phi$, which is composed of a $1 \times 1$ convolution layer, a ReLU activation layer and a $1 \times 1$ convolution layer:
\begin{equation}
\begin{gathered}
PE^K_i = \phi(\overline{V_i}),
\end{gathered}
\end{equation}
where $PE^K_i \in \mathbb{R}^{C \times H_F \times W_F}$ is the 3D position encoding in local coordinates(i.e. camera coordinates), which has the view-invariant property since the variance of camera intrinsic parameters is much smaller than extrinsic parameters. 

Similar to ~\cite{liu2022petrv2}, we use feature-guided position encoder $\Psi$ to incorporate depth-related information provided by 2D image features:
\begin{equation}
\begin{gathered}
K_{geo} = \Psi(F_{2d}) \odot PE^K_i,
\end{gathered}
\end{equation}
where $\Psi$ is composed of a small MLP network and Sigmoid activation layer and $\odot$ is the element-wise multiplication operator. The $K_{geo} \in \mathbb{R}^{C \times H_F \times W_F}$ means the geometric key $K_{geo}$ when calculating the decoupled cross attention.

\textbf{Query Feature-guided Position Encoder.} We initialize a set of 3D reference points $P^L\in \mathbb{R}^{1 * N \times 3}$ in LiDAR 3D space global with uniform distribution. Then we transform the $P^L$ to $P^C \in \mathbb{R}^{S \times N \times 3}$ in camera 3D space via camera extrinsic parameters $R$ and $t$ as:
\begin{equation}
\begin{gathered}
P^C = R \cdot P^L + t,
\end{gathered}
\end{equation}
where $R\in \mathbb{R}^{S \times 3 \times 3}$ is the rotation matrix and $T\in \mathbb{R}^{S \times 3 \times 1}$ is the translation vector from LiDAR to each camera respectively. Then the reference points in camera coordinates are mapped to a high-dimentional sinusoidal position embedding and then fed into a MLP network to get the object position encoding $obj^{pe}$:
\begin{equation}
\begin{gathered}
obj^{pe} = MLP(sinusoidal(P^C))
\end{gathered}
\end{equation}
The position information in $obj^{pe}$ is rather coarse since this embedding is generated from randomly sampled points in 3D space. Thus, we propose Query-feature guided position encoder to incorporate objects' position information. We argue that object queries$Q_{c}$ and object position embedding are in different embedding space, where the former lies in the LiDAR 3D space and the latter lies in the camera 3D space. We use a small MLP network $\Phi$ to project the queries from global embedding space to the local embedding space. Specifically, we get the geometric 3D query $Q_{geo}$(i.e. the refined object position embedding $obj^{pe}_{refine}$) by multiplying $Q_m$ with $obj^{pe}_{coarse}$:
% Hence, the camera extrinsic parameters embedding is generated to achieve the transformation in these two embedding space. Specifically, we first flatten extrinsic parameters $R$ and then projected by a small MLP network $\Phi$ and Sigmoid function$\sigma$. The modulated query $Q_m$ is computed by the element-wise multiplication:
% \begin{equation}
% \begin{gathered}
% Q_m = Q_c \odot \sigma(\Phi(flatten(R)))
% \end{gathered}
% \end{equation}
% The $Q_m$ and $obj^{pe}_{coarse}$ are in the same embedding space. We get the refined object position encoding $obj^{pe}_{refine}$ by multiplying $Q_m$ with $obj^{pe}_{coarse}$:
\begin{equation}
\begin{gathered}
Q_{geo} = obj^{pe} \odot \Phi(Q_c)
\end{gathered}
\end{equation}
% The refined object position embedding is treated as the geometric 3D query $Q_{geo}$ in cross attention mechanism. 

\textbf{Multi-head cross-attention.} Similar to ~\cite{meng2021conditional}, we adopt the standard multi-head decoupled cross attention mechanism. The query is formed by the content query $Q_{c}$ and the geometric query $Q_{geo}$, where $Q_{c}$ is a set of learnable embedding and $Q_{geo}$ is the output from the local object position encoder. The key is accordingly formed by the content key $K_{c}$ and the geometric query $K_{geo}$. The $K_{c}$ is generated as follows:
\begin{equation}
\begin{gathered}
K_{c} = F_{2d} + cam_{emb},
\end{gathered}
\end{equation}
where $cam_{emb}\in \mathbb{R}^{S \times C \times 1 \times 1}$ is the learnable embedding to differentiate different cameras.
The decoupled cross attention could be written as:
\begin{equation}
\begin{gathered}
W = Softmax(\alpha \cdot Q_{c} K_{c}^{T} + \beta \cdot Q_{geo} K_{geo}^{T}), \\
Q_{update} = W \cdot V,
\end{gathered}
\end{equation}
where $\alpha$ and $\beta$ are the weights for content and geometric information respectively. $W$ means affinity map generated by the production of queries and keys. The $Q_{c}$ is updated by the output $Q_{update}$ from decoupled cross attention layer.


\subsection{Temporal Modeling.} 
% lost the process of project reference points to previous frames.
In this section, we illustrate \ourMethod{}-T, the extension of \ourMethod{} with temporal modeling. Since instances may have different positions and poses between frames due to the movement, it is supposed to decompose the queries for capturing instances' geometric information in different frames. Different from warping the BEV feature or encoding the ego motion in the position embedding, we convert 3D reference points to previous frame via the ego motion matrix. Specifically, taking two frames for example, we align the 3D reference points in the current frame to the previous frame as follows:

\begin{equation}
\begin{gathered}
P_{T'}^L = R_{ego} \cdot P_{T}^L + t_{ego},
\end{gathered}
\end{equation}
where $R_{ego}$ represents the rotation matrix of the ego car and $t_{ego}$ represents the transposition matrix. Then spatial queries of each frame are generated by a small MLP described in Sec.\ref{subsection1}. Content queries are shared by frames in the first decoder layer. As shown in Fig.~\ref{fig:temporal}, we send queries on the current frame $Q_T^L$ and queries on the previous frame $Q_{T'}^L$ into the decoder layer $TL^{L}$ separately:
\begin{equation}
\begin{gathered}
O_T^{L+1} = TL^{L}(Q_T^L) \\
O_{T'}^{L+1} = TL^{L}(Q_{T'}^L)
\end{gathered}
\end{equation}
where $O_T^{L+1}$ and $O_{T'}^{L+1}$ are the output queries on the current and previous frame from the $L^{th}$ decoder layer $TL^{L}$separately. We propose a simple temporal fusion block $TF$ to fuse the output queries from the $L^{th}$ decoder layer:
\begin{equation}
\begin{gathered}
Q_T^{L+1}, Q_{T'}^{L+1} = TF(O_T^{L+1}, O_{T'}^{L+1}),
\end{gathered}
\end{equation}
where the output queries $Q_T^{L+1}$ and $Q_{T'}^{L+1}$ from the temporal fusion block are treated as the input queries in the next decoder layer $TL_{L}$. This temporal fusion block is composed of simple MLP operations. A linear projection is firstly used to project each set of queries and then we concatenate them together to generate the attention weights. Then the attention weights are multiplied with queries after another projection layer.


%%%%% Comment end
\end{comment}

% \subsection{Head and Loss.}

